Efficient Sampling in Disease Surveillance through Subpopulations: Sampling Canaries in the Coal Mine

We consider outbreak detection settings of endemic diseases where the population under study consists of various subpopulations available for stratified surveillance. These subpopulations can for example be based on age cohorts, but may also correspond to other subgroups of the population under study such as international travellers. Rather than sampling uniformly across the population, one may elevate the effectiveness of the detection methodology by optimally choosing a sampling subpopulation. We show (under some assumptions) the relative sampling efficiency between two subpopulations is inversely proportional to the ratio of their respective baseline disease risks. This implies one can increase sampling efficiency by sampling from the subpopulation with higher baseline disease risk. Our results require careful treatment of the power curves of exact binomial tests as a function of their sample size, which are non-monotonic due to the underlying discreteness. A case study of COVID-19 cases in the Netherlands illustrates our theoretical findings.

==> notation.tex <==
\RequirePackage{amsthm,amsmath,amsfonts,amssymb,mathtools,bbm}

% Probability notations
\renewcommand{\P}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\Ps}[2]{\mathbb{P}_{#1}\left( #2 \right)}
\newcommand{\Pbig}[1]{\mathbb{P}\big( #1 \big)}
\newcommand{\PBig}[1]{\mathbb{P}\Big( #1 \Big)}
\newcommand{\Pbigg}[1]{\mathbb{P}\bigg( #1 \bigg)}
\newcommand{\PBigg}[1]{\mathbb{P}\Bigg( #1 \Bigg)}
\newcommand{\Pbigs}[2]{\mathbb{P}_{#1}\big( #2 \big)}
\newcommand{\PBigs}[2]{\mathbb{P}_{#1}\Big( #2 \Big)}
\newcommand{\Pbiggs}[2]{\mathbb{P}_{#1}\bigg( #2 \bigg)}
\newcommand{\PBiggs}[2]{\mathbb{P}_{#1}\Bigg( #2 \Bigg)}

\newcommand{\PG}[2]{\mathbb{P}\left(#1 \;\middle\; #2\right)}
\newcommand{\PGs}[3]{\mathbb{P}_{#1}\left( #2 \;\middle\; #3\right)}
\newcommand{\PGbig}[2]{\mathbb{P}\big( #1 \;\big\lvert\; #2\big)}
\newcommand{\PGBig}[2]{\mathbb{P}\Big( #1 \;\Big\lvert\; #2\Big)}
\newcommand{\PGbigg}[2]{\mathbb{P}\bigg( #1 \;\bigg\lvert\; #2\bigg)}
\newcommand{\PGBigg}[2]{\mathbb{P}\Bigg( #1 \;\Bigg\lvert\; #2\Bigg)}
\newcommand{\PGbigs}[3]{\mathbb{P}_{#1}\big( #2 \;\big\lvert\; #3\big)}
\newcommand{\PGBigs}[3]{\mathbb{P}_{#1}\Big( #2 \;\Big\lvert\; #3\Big)}
\newcommand{\PGbiggs}[3]{\mathbb{P}_{#1}\bigg( #2 \;\bigg\lvert\; #3\bigg)}
\newcommand{\PGBiggs}[3]{\mathbb{P}_{#1}\Bigg( #2 \;\Bigg\lvert\; #3\Bigg)}

\newcommand{\Ehn}[1]{\mathbb{E}_{H_0}\left[ #1 \right]}
\newcommand{\Eha}[1]{\mathbb{E}_{H_1}\left[ #1 \right]}
\newcommand{\Var}[1]{\text{Var}\left( #1 \right)}
\newcommand{\Cov}[1]{\text{Cov}\left( #1 \right)}
\newcommand{\Varha}[1]{\text{Var}_{H_1}\left( #1 \right)}
\newcommand{\Covha}[1]{\text{Cov}_{H_1}\left( #1 \right)}
\newcommand{\given}{\;\middle|\;}
\newcommand{\givenbig}{\;\big\lvert\;}
\newcommand{\Given}{\;\lvert\;}

% Expectation notation
\newcommand{\E}[1]{\mathbb{E}\left[ #1 \right]}
\newcommand{\Es}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\Ebig}[1]{\mathbb{E}\big[ #1 \big]}
\newcommand{\EBig}[1]{\mathbb{E}\Big[ #1 \Big]}
\newcommand{\Ebigg}[1]{\mathbb{E}\bigg[ #1 \bigg]}
\newcommand{\EBigg}[1]{\mathbb{E}\Bigg[ #1 \Bigg]}
\newcommand{\Ebigs}[2]{\mathbb{E}_{#1}\big[ #2 \big]}
\newcommand{\EBigs}[2]{\mathbb{E}_{#1}\Big[ #2 \Big]}
\newcommand{\Ebiggs}[2]{\mathbb{E}_{#1}\bigg[ #2 \bigg]}
\newcommand{\EBiggs}[2]{\mathbb{E}_{#1}\Bigg[ #2 \Bigg]}

\newcommand{\EG}[2]{\mathbb{E}\left[#1 \;\middle\; #2\right]}
\newcommand{\EGs}[3]{\mathbb{E}_{#1}\left[ #2 \;\middle\; #3\right]}
\newcommand{\EGbig}[2]{\mathbb{E}\big[ #1 \;\big\lvert\; #2\big]}
\newcommand{\EGBig}[2]{\mathbb{E}\Big[ #1 \;\Big\lvert\; #2\Big]}
\newcommand{\EGbigg}[2]{\mathbb{E}\bigg[ #1 \;\bigg\lvert\; #2\bigg]}
\newcommand{\EGBigg}[2]{\mathbb{E}\Bigg[ #1 \;\Bigg\lvert\; #2\Bigg]}
\newcommand{\EGbigs}[3]{\mathbb{E}_{#1}\big[ #2 \;\big\lvert\; #3\big]}
\newcommand{\EGBigs}[3]{\mathbb{E}_{#1}\Big[ #2 \;\Big\lvert\; #3\Big]}
\newcommand{\EGbiggs}[3]{\mathbb{E}_{#1}\bigg[ #2 \;\bigg\lvert\; #3\bigg]}
\newcommand{\EGBiggs}[3]{\mathbb{E}_{#1}\Bigg[ #2 \;\Bigg\lvert\; #3\Bigg]}

% Limit as n goes to infinity
\newcommand{\ntoinf}{\overset{n\to\infty}{\longrightarrow}}

% Floor, Ceiling, Absolute value and Norm function
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

% Swap the definition of \abs* and \norm*, so that \abs and \norm resizes the size of the brackets, and the starred version does not.
\makeatletter
\let\oldabs\abs
\def\abs{\@ifstar{\oldabs}{\oldabs*}}
\let\oldnorm\norm
\def\norm{\@ifstar{\oldnorm}{\oldnorm*}}
\makeatother

% Limit algebra notations
\newcommand{\bigO}{\ensuremath{\mathcal{O}}}
\newcommand{\bigOp}[1][\mathbb{P}]{\ensuremath{\bigO_{\scriptscriptstyle{}#1}}}
\newcommand{\smallO}{\ensuremath{o}}
\newcommand{\smallOp}[1][\mathbb{P}]{\ensuremath{\smallO_{\scriptscriptstyle{}#1}}}
\newcommand{\smallOmega}{\ensuremath{\omega}}
\newcommand{\smallOmegap}[1][\mathbb{P}]{\ensuremath{\smallOmega_{\scriptscriptstyle{}#1}}}

% Derivative and integration notation, renew command
\renewcommand{\d}{{\rm d}}

% Operators
\DeclareMathOperator*{\argmax}{arg\, max}
\DeclareMathOperator*{\argmin}{arg\, min}

% Stochastic dominance inequalities
\def\lsto{\stackrel{\rm sto}{\leq}}
\def\gsto{\stackrel{\rm sto}{\geq}}

% Other symbols
\renewcommand{\equiv}{\vcentcolon =}
\renewcommand{\exp}[1]{\mathrm{exp}\left(#1\right)}

% Indicator
\newcommand{\ind}[1]{\mathbbm{1}\left\{ #1 \right\}}
\newcommand{\indbig}[1]{\mathbbm{1}\big\{ #1 \big\}}
\newcommand{\indBig}[1]{\mathbbm{1}\Big\{ #1 \Big\}}
\newcommand{\indbigg}[1]{\mathbbm{1}\bigg\{ #1 \bigg\}}
\newcommand{\indBigg}[1]{\mathbbm{1}\Bigg\{ #1 \Bigg\}}

\def\symd{\triangle}

% caligraphic letters
\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% bold letters (upper case)
\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

% bold letters (lower case)
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bd{\mathbf{d}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
\def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

% bold greek letters
\newcommand{\bbeta}{{\boldsymbol\beta}}
\newcommand{\bgamma}{{\boldsymbol\gamma}}
\newcommand{\beps}{{\boldsymbol\eps}}
\newcommand{\bmu}{{\boldsymbol\mu}}
\newcommand{\bxi}{{\boldsymbol\xi}}
\newcommand{\btheta}{{\boldsymbol\theta}}
\newcommand\bSigma{{\boldsymbol\Sigma}}
\newcommand\bOmega{{\boldsymbol\Omega}}
\newcommand\bDelta{{\boldsymbol\Delta}}
\newcommand\bGamma{{\boldsymbol\Gamma}}

% bb letters
\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

% Overline letters (uppercase)
\def\Ab{\overline{A}}
\def\Bb{\overline{B}}
\def\Cb{\overline{C}}
\def\Db{\overline{D}}
\def\Eb{\overline{E}}
\def\Fb{\overline{F}}
\def\Gb{\overline{G}}
\def\Hb{\overline{H}}
\def\Ib{\overline{I}}
\def\Jb{\overline{J}}
\def\Kb{\overline{K}}
\def\Lb{\overline{L}}
\def\Mb{\overline{M}}
\def\Nb{\overline{N}}
\def\Ob{\overline{O}}
\def\Pb{\overline{P}}
\def\Qb{\overline{Q}}
\def\Rb{\overline{R}}
\def\Sb{\overline{S}}
\def\Tb{\overline{T}}
\def\Ub{\overline{U}}
\def\Vb{\overline{V}}
\def\Wb{\overline{W}}
\def\Xb{\overline{X}}
\def\Yb{\overline{Y}}
\def\Zb{\overline{Z}}

% Overline letters (lowercase)
\def\ab{\overline{a}}
\def\bb{\overline{b}}
\def\cb{\overline{c}}
\def\db{\overline{d}}
\def\eb{\overline{e}}
\def\fb{\overline{f}}
\def\gb{\overline{g}}
\def\hb{\overline{h}}
\def\ib{\overline{i}}
\def\jb{\overline{j}}
\def\kb{\overline{k}}
\def\lb{\overline{l}}
\def\mb{\overline{m}}
\def\nb{\overline{n}}
\def\ob{\overline{o}}
\def\pb{\overline{p}}
\def\qb{\overline{q}}
\def\rb{\overline{r}}
%\def\sb{\overline{s}}
\def\tb{\overline{t}}
\def\ub{\overline{u}}
\def\vb{\overline{v}}
\def\wb{\overline{w}}
\def\xb{\overline{x}}
\def\yb{\overline{y}}
\def\zb{\overline{z}}


